LUMA: Low-Dimension Unified Motion Alignment with Dual-Path Anchoring for Text-to-Motion Diffusion Model

While current diffusion-based models, typically built on U-Net architectures, have shown promising results on the text-to-motion generation task, they still suffer from semantic misalignment and kinematic artifacts. Through analysis, we identify severe gradient attenuation in the deep layers of the network as a key bottleneck, leading to insufficient learning of high-level features. To address this issue, we propose \textbf{LUMA} (\textit{\textbf{L}ow-dimension \textbf{U}nified \textbf{M}otion \textbf{A}lignment}), a text-to-motion diffusion model that incorporates dual-path anchoring to enhance semantic alignment. The first path incorporates a lightweight MoCLIP model trained via contrastive learning without relying on external data, offering semantic supervision in the temporal domain. The second path introduces complementary alignment signals in the frequency domain, extracted from low-frequency DCT components known for their rich semantic content. These two anchors are adaptively fused through a temporal modulation mechanism, allowing the model to progressively transition from coarse alignment to fine-grained semantic refinement throughout the denoising process. Experimental results on HumanML3D and KIT-ML demonstrate that LUMA achieves state-of-the-art performance, with FID scores of 0.035 and 0.123, respectively. Furthermore, LUMA accelerates convergence by 1.4$\times$ compared to the baseline, making it an efficient and scalable solution for high-fidelity text-to-motion generation.

==> sec/3_expriment.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/Luma_grad.pdf}
    \caption{\textbf{Gradient magnitudes across network layers in LUMA.} Left: baseline without DAL; Right: with DAL. Red and blue bars denote downsampling and upsampling layers. The dashed line marks the vanishing gradient threshold (1\% of mean). DAL boosts gradients in deep layers, mitigating vanishing issues and enhancing learning.}
    \label{fig:grad_analysis}
\end{figure}
We evaluate our approach on two standard motion-language benchmarks: HumanML3D \cite{Guo_2022_CVPR} and KIT-ML \cite{kit}. HumanML3D contains 14,616 motion sequences from AMASS \cite{AMASS:ICCV:2019} and HumanAct12 \cite{guo2020action2motion}, each paired with three text descriptions (44,970 total), covering diverse actions like walking, exercising, and dancing. KIT-ML includes 3,911 motions and 6,278 descriptions, serving as a smaller-scale benchmark. We follow the standard evaluation protocol of StableMoFusion, including pose representation and mirroring-based augmentation. The data is split into training, validation, and test sets with a ratio of 0.8:0.15:0.05. More details about the datasets and evaluation metrics are available in \textbf{Appendix \ref{ap:Evaluation Metrics}}.
% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{fig/luma_training_plot.png}
%     \caption{
% FID convergence curves for LUMA and the anchor-free baseline (vs. training steps and wall-clock time). The dashed line marks an FID threshold of 0.078. LUMA reaches this in \textbf{35k} iterations (\textbf{1.4$\times$} faster), reducing training time from 8 to \textbf{7 hours}, demonstrating more efficient convergence.
% }
%     \label{fig:fid_curve}
% \end{figure}

\begin{wrapfigure}{l}{0.52\linewidth} % r=靠右；可改 0.45--0.55\linewidth
  \vspace{-6pt}
  \centering
  \includegraphics[width=\linewidth]{fig/luma_training_plot.png}
  \captionsetup{skip=4pt}
  \caption{FID convergence curves for LUMA and the anchor-free baseline (vs. training steps and wall-clock time). The dashed line marks an FID threshold of 0.078. LUMA reaches this in \textbf{35k} iterations (\textbf{1.4$\times$} faster), reducing training time from 8 to \textbf{7 hours}, demonstrating more efficient convergence.}
  \label{fig:fid_curve}
  \vspace{-6pt}
\end{wrapfigure}

% \noindent \textbf{Evaluation metrics.}
% In addition to the commonly utilized metrics such as Frechet Inception Distance (FID) \cite{FID}, R-Precision, Multimodal Distance (MM-Dist), and Diversity, which are employed by StableMoFusion \cite{huang2024stablemofusionrobustefficientdiffusionbased}. Furthermore, human evaluation is employed to obtain accuracy and human preference results for the outputs generated by the model.
% % \end{itemize}

% \begin{itemize}[noitemsep,leftmargin=*]

%     \item \textbf{Frechet Inception Distance  (FID):} We can evaluate the overall motion quality by measuring the distributional difference between the high-level features of the motions. 
%     \item \textbf{R-Precision:} We rank Euclidean distances between a given motion sequence and 32 text descriptions (1 ground-truth and 31 randomly selected mismatched descriptions). We report Top-1, Top-2, and Top-3 accuracy of motion-to-text retrieval. 
    
%     \item \textbf{Diversity:} From a set of motions, we randomly sample 300 pairs and compute the average Euclidean distances between them to measure motion diversity.
%      \item \textbf{Multimodal Distance (MM. Dist.):} measures the degree of alignment between motion and text features; lower values indicate a closer semantic correspondence and stronger cross-modal consistency.
%     \item \textbf{Multimodality (MM.):} For one text description, we generate 20 motion sequences forming 10 pairs of motion. We then extract motion features and compute the average Euclidean distances of the pairs. We finally report the average over all the text descriptions.
    
%     % \item \textbf{Human Evaluation:} We conducted evaluations of each model's generated results in the form of a Google Form. We collected user ratings on model prediction, which encompassed both the quality and correctness of the generated motions. Additionally, we analyzed user preferences for model prediction. Further details will be discussed in Section \ref{sec:human eval} and Appendix C. 
% \end{itemize}
\textbf{Experimental Setup.} We adopt model architecture settings consistent with StableMoFusion \cite{huang2024stablemofusionrobustefficientdiffusionbased}, closely following its training methodology with a total of 50,000 training steps. The diffusion process employs $T=1000$ time steps with a linear beta schedule, and DPM-Solver is used for inference with 10 sampling steps. For DAL, $\lambda_{\text{fre}}$ is set to 0.1, and $\lambda_{\text{tem}}$ is actively used with a value of 0.5. The parameter $k$ is set to 64. In our framework, anchor selection is performed at the Down-block3 stage, where FiLM modulation is also injected. During inference, the classifier-free guidance scale is set to 2.5. A conditional mask probability of 0.1 is applied during training to enable classifier-free guidance. The entire training procedure can be efficiently completed on a single RTX 4090 GPU with 24 GB of memory.


\subsection{Comparison to State-of-the-art Approaches
}

\textbf{Quantitative comparisons.} \label{sec:com_sota}
Following \cite{t2mgpt,guo2023momask}, we report the average over 20 repeated generations with a 95\% confidence interval. Table \ref{tab:human_kit_result}  presents evaluations on the HumanML3D \cite{Guo_2022_CVPR} and KIT-ML \cite{kit} datasets, respectively, in comparison with state-of-the-art (SOTA) approaches.

\input{tab/main_exam}

In terms of empirical results, LUMA demonstrates strong performance across all key evaluation metrics. Our method achieves substantial improvements in FID (HumanML3D: \textbf{0.035}; KIT: \textbf{0.123}) and R-Precision (Top-3 HumanML3D: \textbf{0.839}; KIT: \textbf{0.796}), clearly illustrating the effectiveness of LUMA in enhancing the baseline model. Compared to state-of-the-art VQ-based approaches such as MMM \cite{pinyoanuntapong2024mmmgenerativemaskedmotion} and MoMask \cite{guo2023momask}, LUMA consistently achieves competitive or superior results on the HumanML3D dataset, outperforming other methods in terms of FID, R-Precision, and MultiModal Distance. This highlights LUMA’s ability to generate high-quality, semantically aligned, and diverse motion sequences. On the more challenging KIT-ML benchmark, LUMA attains the best FID among all evaluated methods and ranks first in R-Precision, demonstrating the broad adaptability of the LUMA architecture. Overall, these results underscore the capability of LUMA to significantly improve both the quality and diversity of text-driven motion generation.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/motions.pdf}
    \caption{Visualization Comparison. We compare the visual results of LUMA with three state-of-the-art methods. In both examples, LUMA consistently produces more accurate, natural, and fine-grained motion than the other approaches.}
    \label{fig:visualization}
\end{figure}

\textbf{Qualitative comparison.} 
Figure~\ref{fig:visualization} presents visual comparisons with MDM, StableMoFusion, and MoMask under three prompts. For "A man crouched down and then rolled forward," MDM and StableMoFusion only crouch, while MoMask fails to roll properly. Our model performs the full action accurately. For "A person kneels down onto the floor then waits and raises his hands up," MDM misses kneeling, and others raise hands poorly; our method captures both with correct timing. For the complex prompt involving hand-raising and circling, baselines fail to complete all sub-actions, while our model executes them with high fidelity. These results demonstrate superior semantic understanding, temporal consistency, and detail accuracy.

%提高模型收敛速度
\subsection{Faster Convergence with Dual Anchors}
As shown in Figure~\ref{fig:fid_curve}, LUMA achieves significantly faster convergence compared to the anchor-free baseline. Our model surpasses the FID threshold of 0.078 with only \textbf{35k} training iterations, whereas the baseline requires \textbf{50k} steps, resulting in a \textbf{1.4$\times$} speedup. This efficiency gain is also reflected in the wall-clock training time. As illustrated on the upper axis of the same figure, LUMA reaches the target FID in just \textbf{7 hours}, while the baseline takes \textbf{8 hours}. This demonstrates that our dual-anchor alignment not only improves motion quality but also makes training substantially more efficient, both in computation steps and real-world time.
%梯度分析

%鲁棒性分析

\subsection{Gradient Analysis}
As shown in Figure~\ref{fig:grad_analysis}, removing the DAL causes the gradient magnitudes in the middle layers to drop sharply. The downsampling path is especially affected. Some layers fall below the vanishing threshold (1\% of the mean). This indicates severe gradient attenuation in these regions. After introducing the DAL, the gradients in the deep downsampling layers increase by nearly two orders of magnitude and are brought to a level comparable with the upsampling path. This observation validates our earlier hypothesis that vanishing gradients in deep layers hinder effective learning of abstract features. The additional semantic and motion anchors introduced by DAL provide more informative supervisory signals to the encoder, substantially alleviating the vanishing gradient problem and accelerating effective representation learning in deeper layers.




\subsection{Ablation Study}

To comprehensively assess the contribution of each component in our framework, we conduct a series of controlled ablation experiments. Following the evaluation protocol, we focus on two aspects: (i) the effect of each core module, (ii) the influence of key design choices. All experiments are performed under identical training settings for fair comparison.

\textbf{Core Component Analysis.} As shown in Table~\ref{tab:core_components}, each component of LUMA plays a critical and complementary role. The backbone alone achieves a baseline FID of 0.152, while removing both anchors but retaining the LUMA architecture already yields a substantial FID drop to 0.067, highlighting structural benefits. Introducing either the frequency semantic or temporal semantic anchor alone further reduces FID to 0.057 and improves R@3 to 0.840, indicating that both anchors independently enhance motion quality and text alignment. Their similar contributions suggest that each focuses on a different aspect of the generation process. One captures frequency-level structure, while the other improves semantic consistency. Removing MoCLIP leads to a slight drop in performance, confirming its importance in providing effective semantic supervision. Meanwhile, eliminating FiLM leads to a marginal drop in R@3 despite strong FID, showing its importance in temporal modulation. The full model outperforms all variants (FID 0.035, R@3 0.839), demonstrating that these modules act synergistically to improve fidelity, semantic alignment, and training stability.

\input{tab/core_components}

\input{tab/design_choices}
\input{tab/anchor_weighting}

% \textbf{Design Choice Exploration.} We systematically investigate the impact of two critical hyperparameters in LUMA: the number of retained DCT coefficients ($k$) for frequency semantic anchoring, and the FiLM modulation injection location. As reported in Table~\ref{tab:design_choices}, setting $k$ to an intermediate value ($k=64$) achieves the best balance between preserving global motion structure and suppressing high-frequency noise. Both lower ($k=8$) and higher ($k=128$) values result in inferior performance, either limiting expressiveness or introducing excessive artifacts. For FiLM injection, positioning the modulation at Down-block3 yields the most favorable trade-off, capturing sufficient temporal context without incurring the loss of fine details or increasing computational burden, as observed with shallower or deeper placements.

% To rigorously assess the effectiveness of the proposed dynamic anchor weighting strategy, we compare it with two alternatives: (i) \emph{static averaging}, where anchor weights are held constant during training, and (ii) \emph{fixed learnable weights}, which are treated as global trainable parameters. Table~\ref{tab:anchor_weighting} demonstrates that the dynamic cosine-annealed schedule consistently outperforms both baselines, delivering the best FID and R@3 scores. This adaptive approach enables the model to emphasize temporal semantic and frequency semantic alignment in the early training phases while gradually relaxing these constraints, thereby preventing over-regularization and allowing finer motion refinement in later stages. These results validate the design motivation for dynamic scheduling and highlight its essential role in optimizing both the fidelity and semantic consistency of generated motions.

\textbf{Design Choice Exploration.}
We study two key hyperparameters in LUMA: the number of retained DCT coefficients ($k$) and the FiLM injection location.
As shown in Table \ref{design_choice}, an intermediate setting ($k=64$) best balances global structure and noise suppression; smaller ($k=8$) limits expressiveness, while larger ($k=128$) introduces artifacts.
For FiLM, injecting at \textit{Down-block3} provides the best trade-off, capturing sufficient temporal context without losing fine details or adding notable compute.

\textbf{Dynamic Anchor Weighting.}
We compare our dynamic cosine-annealed schedule with (i) \emph{static averaging} and (ii) \emph{fixed learnable weights}.
Table~\ref{tab:anchor_weighting} shows the dynamic scheme consistently achieves the best FID and R@3.
It emphasizes temporal and frequency alignment early, then gradually relaxes constraints to avoid over-regularization, enabling finer motion refinement and stronger semantic consistency.


% \paragraph{Efficiency Analysis}  
% To evaluate the practicality of our approach, we report parameter count, training time, and inference speed for each variant. As presented in Table~\ref{tab:efficiency}, the introduction of our modules incurs minimal additional computational overhead, maintaining competitive resource efficiency while achieving significant performance gains.

% %\input{tab/efficiency}







==> sec/fake.tex <==
\begin{algorithm}[ht]
\caption{LUMA Training}
\label{alg:luma}
\KwIn{$\mathcal{D}$; Encoders $f_{\text{text}},f_{\text{tem}}$; Params $\Theta$; Hyperparams $(k,\lambda_{\text{fre}},\lambda_{\text{tem}},N,T)$}
\KwOut{$\Theta$}

\For{$n=1$ \KwTo $N_{\text{train}}$}{
    Sample $(\mathbf{x}_0,\mathbf{c})$, $t\sim\mathcal{U}[1,T]$, $\epsilon\sim\mathcal{N}(0,I)$\;
    $\mathbf{x}_t=\sqrt{\alpha_t}\mathbf{x}_0+\sqrt{1-\alpha_t}\epsilon$\;
    $(\hat{\epsilon},\mathbf{h})=\mathcal{D}_{\phi}(\mathbf{x}_t,f_{\text{text}}(\mathbf{c}),t)$\;
    $(\mathbf{z}_f,\mathbf{z}_t)=\textsf{ANCHOR}_{\theta,\psi,\psi'}(\mathbf{h},t)$\;
    $\omega=\frac{1}{2}[1+\cos(\pi\min(\frac{n}{N},1))]$\;
    $\mathcal{L}=\|\hat{\epsilon}-\epsilon\|_2^2+\omega(\lambda_{\text{fre}}\|\mathbf{z}_f-\mathrm{DCT}_k(\mathbf{x}_0)\|_2^2+\lambda_{\text{tem}}(1-\cos(\mathbf{z}_t,f_{\text{tem}}(\mathbf{x}_0))))$\;
    Update $\Theta$ via $\nabla_{\Theta}\mathcal{L}$\;
}
\end{algorithm}


==> tab/humanml3d.tex <==
\begin{table*}[t]
\centering
%\resizebox{\textwidth}{!}{%
%\footnotesize
\begin{tabular}{llccccccc}
\toprule
\textbf{Method} & \textbf{Venue} & \textbf{FID $\downarrow$}  &\multicolumn{3}{c}{\textbf{R-Precision $\uparrow$}} & \textbf{Diversity $\rightarrow$}  & \textbf{MM. Dist.$\downarrow$} & \textbf{MM. $\uparrow$}\\ \cmidrule(lr){4-6}
 &  &  & \textbf{Top1} & \textbf{Top2} & \textbf{Top3} & & & \\ \midrule
\multicolumn{9}{c}{\textbf{HumanML3D}} \\ \midrule
Real  &  - & $0.002^{\pm.000}$ & $0.511^{\pm.003}$ & $0.703^{\pm.003}$ & $0.797^{\pm.002}$ & $9.503^{\pm.065}$ & - & -\\
MLD (\citeauthor{chen2023executingcommandsmotiondiffusion}) & CVPR 2023   & $0.473^{\pm.013}$ & $0.481^{\pm.003}$ & $0.673^{\pm.003}$ & $0.772^{\pm.002}$ & $9.724^{\pm.082}$& $3.196^{\pm.010}$ & $\underline{2.413}^{\pm.079}$\\
ReMoDiffuse (\citeauthor{zhang2023remodiffuse}) & ICCV 2023 & $0.103^{\pm.004}$ & $0.510^{\pm.005}$ & $0.698^{\pm.006}$ & $0.795^{\pm.004}$ & $9.018^{\pm.075}$ & ${3.025}^{\pm.008}$ & $1.795^{\pm.043}$\\
MotionDiffuse (\citeauthor{zhang2024motiondiffuse}) & TPAMI 2024 & $0.630^{\pm.001}$ & $0.491^{\pm.001}$ & $0.681^{\pm.001}$ & $0.782^{\pm.001}$ & $9.410^{\pm.049}$ & $3.113^{\pm.001}$ & $1.553^{\pm.042}$\\
MotionLCM (\citeauthor{dai2024motionlcmrealtimecontrollablemotion}) & ECCV 2024 & $0.467^{\pm.012}$ & $0.502^{\pm.003}$ & $0.701^{\pm.002}$ & $0.803^{\pm.002}$ & $9.361^{\pm.660}$ &$3.012^{\pm.007}$ &$2.172^{\pm.082}$\\
T2M-GPT (\citeauthor{t2mgpt}) & CVPR 2023 & $0.141^{\pm.005}$ & $0.492^{\pm.003}$ & $0.679^{\pm.002}$ & $0.775^{\pm.002}$ & $9.722^{\pm.082}$ & $3.121^{\pm.009}$ &$1.831^{\pm.048}$\\
MotionGPT (\citeauthor{jiang2023motiongpthumanmotionforeign}) & NeurIPS 2023 & ${0.232}^{\pm.008}$ & ${0.492}^{\pm.003}$ & ${0.681}^{\pm.003}$ & ${0.778}^{\pm.002}$ & ${9.528}^{\pm.071}$ & ${3.096}^{\pm.008}$ & ${2.008}^{\pm.084}$ \\
MMM (\citeauthor{pinyoanuntapong2024mmmgenerativemaskedmotion})& CVPR 2024 & $0.089^{\pm.002}$ & $0.515^{\pm.002}$ & $0.708^{\pm.002}$ & $0.804^{\pm.002}$& $9.577^{\pm.050}$ &$2.926^{\pm.007}$ &$1.226^{\pm.035}$\\
MoMask (\citeauthor{guo2023momask})& CVPR 2024 & $\underline{0.045}^{\pm.002}$ & $0.521^{\pm.002}$ & $0.713^{\pm.002}$ & $0.807^{\pm.002}$& - & ${2.958}^{\pm.008}$ & $1.241^{\pm.040}$\\
MDM (\citeauthor{mdm}) & ICLR 2023   & $0.544^{\pm.044}$ & $0.320^{\pm.005}$ & $0.498^{\pm.004}$ & $0.611^{\pm.007}$ & $\underline{9.559}^{\pm.086}$ &$5.556^{\pm.027}$ &$\textbf{2.799}^{\pm.072}$ \\
StableMoFusion (\citeauthor{huang2024stablemofusionrobustefficientdiffusionbased}) & ACM MM 2024 & $0.152^{\pm.004}$ & $\underline{0.546}^{\pm.002}$ & $\underline{0.742}^{\pm.002}$ &$\underline{0.835}^{\pm.002}$ & $\textbf{9.466}^{\pm.002}$
&$\underline{2.781}^{\pm.011}$ &$1.362^{\pm.062}$\\ 

LUMA (Ours) & - & $\textbf{0.035}^{\pm.002}$ & $\textbf{0.556}^{\pm.003}$ & $\textbf{0.750}^{\pm.002}$ & $\textbf{0.839}^{\pm.0013}$ & ${9.596}^{\pm.083}$ & $\textbf{2.763}^{\pm.008}$ & ${1.696}^{\pm.049}$ \\
\midrule
\multicolumn{9}{c}{\textbf{KIT-ML}} \\ \midrule
Ground Truth & - & $0.031^{\pm.004}$ & $0.424^{\pm.005}$ & $0.649^{\pm.006}$ & $0.779^{\pm.006}$ & $11.080^{\pm.097}$ & - & - \\
MLD (\citeauthor{chen2023executingcommandsmotiondiffusion}) & CVPR 2023 & ${0.404}^{\pm.027}$ & ${0.390}^{\pm.008}$ & ${0.609}^{\pm.008}$ & ${0.734}^{\pm.007}$ & ${10.800}^{\pm.117}$ & ${3.204}^{\pm.027}$ & $\underline{2.192}^{\pm.071}$\\
ReMoDiffuse (\citeauthor{zhang2023remodiffuse}) & ICCV 2023 & ${0.155}^{\pm.006}$ & ${0.427}^{\pm.014}$ & ${0.641}^{\pm.004}$ & ${0.765}^{\pm.055}$ & ${10.800}^{\pm.105}$ & $2.814^{\pm.028}$ & $1.239^{\pm.028}$ \\
MotionDiffuse (\citeauthor{zhang2024motiondiffuse}) & TPAMI 2024  & ${1.954}^{\pm.062}$ & ${0.417}^{\pm.004}$ & ${0.621}^{\pm.004}$ & ${0.739}^{\pm.004}$ & $\textbf{11.100}^{\pm.143}$ & ${2.958}^{\pm.005}$ & ${0.730}^{\pm.013}$ \\
T2M-GPT (\citeauthor{t2mgpt}) & CVPR 2023 & ${0.514}^{\pm.029}$ & ${0.416}^{\pm.006}$ & ${0.627}^{\pm.006}$ & ${0.745}^{\pm.006}$ & ${10.921}^{\pm.108}$ & ${3.007}^{\pm.023}$ & ${1.570}^{\pm.039}$ \\
MotionGPT (\citeauthor{jiang2023motiongpthumanmotionforeign}) & NeurIPS 2023 & ${0.510}^{\pm.016}$ & ${0.366}^{\pm.005}$ & ${0.558}^{\pm.004}$ & ${0.680}^{\pm.005}$ & ${10.350}^{\pm.084}$ & ${3.527}^{\pm.021}$ & $\textbf{2.328}^{\pm.117}$ \\
MMM (\citeauthor{pinyoanuntapong2024mmmgenerativemaskedmotion})& CVPR 2024& ${0.316}^{\pm.028}$ & ${0.404}^{\pm.005}$ & ${0.621}^{\pm.005}$ & ${0.744}^{\pm.004}$ & ${10.910}^{\pm.101}$ & $2.977^{\pm.019}$ & $1.232^{\pm.039}$ \\
MoMask (\citeauthor{guo2023momask})& CVPR 2024 & $\underline{0.204}^{\pm.011}$ & ${0.433}^{\pm.007}$ & ${0.656}^{\pm.005}$ & ${0.781}^{\pm.005}$ & - & ${2.779}^{\pm.022}$ & ${1.131}^{\pm.043}$ \\
MDM (\citeauthor{mdm}) & ICLR 2023 & ${0.497}^{\pm.021}$ & ${0.164}^{\pm.004}$ & ${0.291}^{\pm.004}$ & ${0.396}^{\pm.004}$ & ${10.847}^{\pm.119}$ & ${9.191}^{\pm.022}$ & ${1.907}^{\pm.214}$ \\
StableMoFusion (\citeauthor{huang2024stablemofusionrobustefficientdiffusionbased}) & ACM MM 2024 & ${0.258}^{\pm.029}$ & $\underline{0.446}^{\pm.006}$ &$\underline{0.660}^{\pm.005}$ & $\underline{0.782}^{\pm.004}$ & $\underline{10.936}^{\pm.077}$ & $\underline{2.800}^{\pm.018}$ & ${1.362}^{\pm.062}$ \\
LUMA (Ours) & - &\textbf{ ${0.123}^{\pm.014}$ }& $\textbf{0.454}^{\pm.006}$& $\textbf{0.675}^{\pm.005}$ & $\textbf{0.796}^{\pm.005}$ & ${10.803}^{\pm.076}$ & $\textbf{2.711}^{\pm.015}$ & ${1.233}^{\pm.055}$ \\
\bottomrule
\end{tabular}%
%}

\caption{Experimental results on HumanML3D and KIT-ML datasets. $\pm$ indicates a 95\% confidence interval. \textbf{Bold} and \underline{Underline} indicate the best and the second-best results, respectively. The right arrow ($\rightarrow$) denotes that a higher value is closer to real motion. Our method achieves state-of-the-art FID and R-Precision across both benchmarks.
}
\label{tab:human_kit_result}
\end{table*}

